Audio-Visual Class-Incremental Learning for Fish Feeding intensity Assessment in Aquaculture

Fish Feeding Intensity Assessment (FFIA) is crucial in industrial aquaculture management. Recent multi-modal approaches have shown promise in improving FFIA robustness and efficiency. However, these methods face significant challenges when adapting to new fish species or environments due to catastrophic forgetting and the lack of suitable datasets. To address these limitations, we first introduce AV-CIL-FFIA, a new dataset comprising 81,932 labelled audio-visual clips capturing feeding intensities across six different fish species in real aquaculture environments. Then, we pioneer audio-visual class incremental learning (CIL) for FFIA and demonstrate through benchmarking on AV-CIL-FFIA that it significantly outperforms single-modality methods. Existing CIL methods rely heavily on historical data. Exemplar-based approaches store raw samples, creating storage challenges, while exemplar-free methods avoid data storage but struggle to distinguish subtle feeding intensity variations across different fish species. To overcome these limitations, we introduce HAIL-FFIA, a novel audio-visual class-incremental learning framework that bridges this gap with a prototype-based approach that achieves exemplar-free efficiency while preserving essential knowledge through compact feature representations. Specifically, HAIL-FFIA employs hierarchical representation learning with a dual-path knowledge preservation mechanism that separates general intensity knowledge from fish-specific characteristics. Additionally, it features a dynamic modality balancing system that adaptively adjusts the importance of audio versus visual information based on feeding behaviour stages. Experimental results show that HAIL-FFIA is superior to SOTA methods on AV-CIL-FFIA, achieving higher accuracy with lower storage needs while effectively mitigating catastrophic forgetting in incremental fish species learning.

==> text/S4.benckmark.tex <==
\section{Benchmark Studies on audio and visual CIL}
\label{sec:benchmark}

\subsection{Audio-based CIL for FFIA}
\subsubsection{Learning without Forgetting (LwF)}
Learning without Forgetting (LwF) \cite{li2017learning} is a prominent approach in class incremental learning that aims to preserve knowledge of previously learned tasks while learning new ones. In the context of audio-based CIL for FFIA, we adapt LwF to handle sequential learning of new fish species or feeding intensities.
The core idea of LwF is to use knowledge distillation to transfer knowledge from the old model to the new one. Initially, we train a model $\theta_{old}$ on the initial set of classes (fish species or feeding intensities) using the audio data. When new classes are introduced, we initialize a new model $\theta_{new}$ with the weights of $\theta_{old}$.

For each new training sample $x$, we compute two sets of outputs: $y_{old} = \theta_{old}(x)$, which are the predictions of the old model, and $y_{new} = \theta_{new}(x)$, which are the predictions of the new model.
The total loss $L_{total}$ is a combination of two components:

\begin{equation}
L_{total} = \lambda L_{new} + (1-\lambda) L_{old}
\end{equation}

Here, $L_{new}$ is the standard cross-entropy loss for new classes, $L_{old}$ is the knowledge distillation loss (typically KL divergence) between $y_{old}$ and $y_{new}$ for old classes, and $\lambda$ is a hyperparameter balancing the two loss components. We update $\theta_{new}$ by minimizing $L_{total}$ using standard optimization techniques.
% In our audio-based FFIA implementation, we apply LwF to the audio feature extraction network. The audio data is first transformed into mel-spectrograms, which serve as input to a convolutional neural network. As new fish species or feeding intensities are introduced, LwF helps maintain performance on previously learned classes while adapting to new ones.

\subsubsection{Elastic Weight Consolidation (EWC)}

Elastic Weight Consolidation (EWC) \cite{kirkpatrick2017overcoming} is another prominent approach in class incremental learning that aims to mitigate catastrophic forgetting. In the context of audio-based CIL for FFIA, we adapt EWC to preserve knowledge about previously learned fish species or feeding intensities while learning new ones.

EWC operates on the principle that some parameters in a neural network are more important for certain tasks than others. It attempts to keep the parameters close to their optimal values for previously learned tasks while allowing them to adapt to new tasks. This is achieved by adding a regularization term to the loss function.

The EWC loss function is defined as:

\begin{equation}
L(\theta) = L_{new}(\theta) + \sum_i \frac{\lambda}{2} F_i (\theta_i - \theta_{A,i}^*)^2
\end{equation}

Where:
 $L_{new}(\theta)$ is the loss for the new task, $\lambda$ is a hyperparameter that determines the importance of the old task, $F_i$ is the Fisher information matrix, which measures the importance of parameter $i$ for the old task
, $\theta_{A,i}^*$ is the optimal parameter value for the old task


% In our audio-based FFIA implementation, we apply EWC to the entire audio processing network. When new fish species or feeding intensities are introduced, we compute the Fisher information matrix on the old task's validation set. This matrix helps identify which weights in the network are crucial for recognizing previously learned species or intensities.
% As we train on new classes, the EWC regularization term encourages the model to keep important weights close to their previous values, while allowing less important weights to change more freely. This approach enables the model to learn new audio patterns associated with new fish species or feeding intensities while retaining its ability to recognize patterns from previously learned classes.
% EWC offers a more flexible approach compared to LwF, as it allows for finer control over which parts of the model are preserved. However, additional computation is required to calculate the Fisher information matrix, and its effectiveness may decrease as the number of tasks grows, especially if there are significant differences between the audio characteristics of different fish species.


\subsubsection{Independent Learning with Output and Feature Discrepancy (IODFD)}

IODFD \cite{mulimani2024class} is a novel approach that combines Independent Learning (IndL) with Output Discrepancy (OD) and Feature Discrepancy (FD) to address class-incremental learning challenges in audio-based FFIA. This method aims to balance learning new classes while preserving knowledge of previously learned ones.

For each new training sample $x$, we compute three key outputs:

\begin{equation}
y_{new} = \sigma(H^i_\phi(F^i_\theta(x))_{new})
\end{equation}

This represents the predictions for new classes, where $\sigma$ is the sigmoid function, $H^i_\phi$ is the current classifier, and $F^i_\theta$ is the current feature extractor.

\begin{equation}
o_{old} = H^i_\phi(F^i_\theta(x))_{old}
\end{equation}

This represents the logits for old classes from the current model.

\begin{equation}
\hat{o}_{old} = \hat{H}^{i-1}_\phi(\hat{F}^{i-1}_\theta(x))_{old}
\end{equation}

This represents the logits for old classes from the frozen previous model.

The total loss function combines three components:

\begin{equation}
L_{total} = L_{BCE} + L_{FD} + \lambda L_{OD}
\end{equation}

Where:

$L_{BCE}$ is the binary cross-entropy loss for new classes, encouraging the model to learn new patterns.

$L_{FD}$ is the feature discrepancy loss, which helps preserve feature representations of old classes:

\begin{equation}
L_{FD} = 1 - \cos(\text{norm}(\hat{F}^{i-1}_\theta(x)), \text{norm}(F^i_\theta(x)))
\end{equation}

$L_{OD}$ is the output discrepancy loss, which maintains consistent outputs for old classes:

\begin{equation}
L_{OD} = D_{KL}(\pi(\hat{o}_{old}) || \pi(o_{old}))
\end{equation}

Here, $D_{KL}$ is the Kullback-Leibler divergence, and $\pi$ is a temperature-scaled softmax function:

\begin{equation}
\pi(u) = u^{1/\Delta} / \sum_j u_j^{1/\Delta}
\end{equation}
The value of $\Delta$ is set to higher than 1 to increase the weights of smaller values. 
$\lambda$ is an adaptive weight that increases as the number of classes grows:

\begin{equation}
\lambda = \Omega\sqrt{|C|/|C_{new}|}
\end{equation}

Where $\Omega$ is a fixed constant, $|C|$ is the total number of classes, and $|C_{new}|$ is the number of new classes.

% By combining these components, IODFD enables the FFIA system to learn new audio patterns while mitigating catastrophic forgetting of previously learned ones. This approach addresses the stability-plasticity dilemma by preserving old knowledge at both the feature and output levels while allowing flexibility to learn new classes.





% \subsubsection{other}
% Compared with Xubo-replay-based CL (RCL), Manjunath Mulimani-independent learning (IndL), LwF, fine-tuning (FT), feature extraction (FE),





\subsection{Visual-based CIL for FFIA}

\subsubsection{Incremental Classifier and Representation Learning (iCaRL)}

iCaRL is a prominent approach in class-incremental learning that combines representation learning with nearest-exemplar classification. For visual-based FFIA, we adapt iCaRL to handle sequential learning of new fish species or feeding intensities while maintaining performance on previously learned classes.

For each new training sample $x$, we compute:

\begin{equation}
y = \sigma(F_\theta(x))
\end{equation}

Here, $F_\theta$ is the feature extractor with parameters $\theta$, and $\sigma$ is the sigmoid activation function.

The loss function combines classification loss and distillation loss:

\begin{equation}
L_{\text{total}} = L_{\text{classify}} + \lambda L_{\text{distill}}
\end{equation}

\begin{equation}
L_{\text{classify}} = -\sum_{k=1}^{|C|} y_k \cdot \log(\hat{y}_k) + (1 - y_k) \cdot \log(1 - \hat{y}_k)
\end{equation}

\begin{equation}
L_{\text{distill}} = \sum_{k \in C_{\text{old}}} \hat{y}_k^{\text{old}} \log(\hat{y}_k) + (1 - \hat{y}_k^{\text{old}}) \log(1 - \hat{y}_k)
\end{equation}

In these equations, $|C|$ is the total number of classes, $y_k$ is the ground truth for class $k$, $\hat{y}_k$ is the predicted probability for class $k$, $C_{\text{old}}$ is the set of old classes, $\hat{y}_k^{\text{old}}$ is the output of the previous model for old class $k$, and $\lambda$ is a balancing parameter.

After each incremental phase, iCaRL updates its exemplar set $P$ by selecting $m$ examples per class that best approximate the class mean in the feature space:

\begin{equation}
\mu_c = \frac{1}{|X_c|} \sum_{x \in X_c} F_\theta(x)
\end{equation}

\begin{equation}
P_c = \argmin_{P:|P|=m} \|\mu_c - \frac{1}{|P|} \sum_{x \in P} F_\theta(x)\|
\end{equation}

Here, $\mu_c$ is the mean feature vector for class $c$, $X_c$ is the set of all examples for class $c$, $P_c$ is the exemplar set for class $c$, and $m$ is the number of exemplars per class.

During inference, iCaRL uses a nearest-mean-of-exemplars classification rule:

\begin{equation}
\hat{c} = \argmin_c \|F_\theta(x) - \mu_c\|
\end{equation}

Where $\hat{c}$ is the predicted class and $x$ is the input sample.


\subsubsection{Learning a Unified Classifier Incrementally via Rebalancing (UCIR)}

UCIR is an effective approach to class-incremental learning that addresses the issue of classifier bias towards newly learned classes. For visual-based FFIA, we adapt UCIR to effectively learn new fish species or feeding intensities while maintaining performance on previously learned classes.

The core idea of UCIR is to use a cosine normalization-based classifier and employ a rebalancing strategy. For each input image $x$, the feature extractor $f_\theta$ produces a feature vector, which is then normalized:

\begin{equation}
\hat{v} = \frac{f_\theta(x)}{\|f_\theta(x)\|}
\end{equation}

The classifier's weight vectors are also normalized, resulting in the following classification score for class $k$:

\begin{equation}
s_k = \eta \cdot \frac{w_k^T \hat{v}}{\|w_k\|}
\end{equation}

Here, $\eta$ is a learnable scaling factor, and $w_k$ is the weight vector for class $k$.

The loss function in UCIR combines two main components:

\begin{equation}
L_{\text{total}} = L_{\text{CB}} + \lambda L_{\text{distill}}
\end{equation}

$L_{\text{CB}}$ is the class-balanced cross-entropy loss that addresses the data imbalance between old and new classes:

\begin{equation}
L_{\text{CB}} = -\frac{1}{|C|} \sum_{k=1}^{|C|} \frac{\beta_k}{1-\beta_k} \log p_k
\end{equation}

Where $\beta_k = (N/n_k)^{1/4}$, $N$ is the total number of samples, $n_k$ is the number of samples for class $k$, and $p_k$ is the predicted probability for class $k$.

$L_{\text{distill}}$ is a less-forget constraint that uses cosine similarity to preserve old class knowledge:

\begin{equation}
L_{\text{distill}} = 1 - \frac{1}{|C_{\text{old}}|} \sum_{k \in C_{\text{old}}} \cos(f_\theta(x), f_{\theta'}(x))
\end{equation}

Where $f_{\theta'}$ is the feature extractor from the previous phase, and $C_{\text{old}}$ is the set of old classes.

During inference, UCIR employs a rebalancing strategy to adjust the classifier outputs:

\begin{equation}
\hat{s}_k = 
\begin{cases} 
s_k \cdot (1 - \alpha_t) + \alpha_t & \text{if } k \in C_{\text{old}} \\
s_k \cdot (1 - \alpha_t) & \text{if } k \in C_{\text{new}}
\end{cases}
\end{equation}

Here, $\alpha_t = t / T$ where $t$ is the current incremental step and $T$ is the total number of steps.

\subsubsection{Pooled Outputs Distillation Network (PODNet)}

PODNet is an advanced approach to class-incremental learning that addresses the challenges of catastrophic forgetting and feature drift. For visual-based FFIA, we adapt PODNet to effectively learn new fish species or feeding intensities while maintaining performance on previously learned classes.

The core idea of PODNet is to use a multi-scale feature distillation loss and a pooled classifier. For an input image $x$, the feature extractor $f_\theta$ produces feature maps at multiple scales:

\begin{equation}
F = \{f_\theta^l(x) | l \in L\}
\end{equation}

Where $L$ is the set of selected layers for feature distillation.

The multi-scale feature distillation loss is defined as:

\begin{equation}
L_{\text{POD}} = \sum_{l \in L} \| \text{POD}(f_\theta^l(x)) - \text{POD}(f_{\theta'}^l(x)) \|_2^2
\end{equation}

Here, $f_{\theta'}$ is the feature extractor from the previous phase, and POD is the pooled output distillation operation:

\begin{equation}
\text{POD}(f) = [\text{GAP}(f), \text{GMP}(f)]
\end{equation}

Where GAP and GMP are global average pooling and global max pooling, respectively.

The classification is performed using a cosine similarity-based classifier:

\begin{equation}
s_k = \eta \cdot \frac{w_k^T \hat{v}}{\|w_k\| \|\hat{v}\|}
\end{equation}

Where $\hat{v}$ is the normalized feature vector, $w_k$ is the weight vector for class $k$, and $\eta$ is a learnable scaling factor.

The total loss function in PODNet combines classification loss and distillation loss:

\begin{equation}
L_{\text{total}} = L_{\text{CE}} + \lambda L_{\text{POD}}
\end{equation}

$L_{\text{CE}}$ is the standard cross-entropy loss, and $\lambda$ is a balancing parameter.

To mitigate class imbalance during incremental learning, PODNet employs a memory bank $M$ of exemplars from old classes. During training, mini-batches are constructed by sampling equally from new class data and the memory bank.


